HyScale-GNN: A Scalable Hybrid GNN Training System on Single-Node Heterogeneous Architecture

Graph Neural Networks (GNNs) have shown success in many real-world applications that involve graph-structured data. Most of the existing single-node GNN training systems are capable of training medium-scale graphs with tens of millions of edges; however, scaling them to large-scale graphs with billions of edges remains challenging. In addition, it is challenging to map GNN training algorithms onto a computation node as state-of-the-art machines feature heterogeneous architecture consisting of multiple processors and a variety of accelerators. We propose HyScale-GNN, a novel system to train GNN models on a single-node heterogeneous architecture. HyScale- GNN performs hybrid training which utilizes both the processors and the accelerators to train a model collaboratively. Our system design overcomes the memory size limitation of existing works and is optimized for training GNNs on large-scale graphs. We propose a two-stage data pre-fetching scheme to reduce the communication overhead during GNN training. To improve task mapping efficiency, we propose a dynamic resource management mechanism, which adjusts the workload assignment and resource allocation during runtime. We evaluate HyScale-GNN on a CPU-GPU and a CPU-FPGA heterogeneous architecture. Using several large-scale datasets and two widely-used GNN models, we compare the performance of our design with a multi-GPU baseline implemented in PyTorch-Geometric. The CPU-GPU design and the CPU-FPGA design achieve up to 2.08x speedup and 12.6x speedup, respectively. Compared with the state-of-the-art large-scale multi-node GNN training systems such as P3 and DistDGL, our CPU-FPGA design achieves up to 5.27x speedup using a single node.

==> 4_hardware.tex <==
%Maybe go from an optimization point of view
\subsection{Hardware Mapping}
Mention which part of the GNN training is done on the FPGA and why. 
Then, show how are these computations mapped to hardware kernels.

\subsection{Data Layout}
Introduce the COO format

\subsection{Optimizations}
Explain the bottleneck of GNN training, and the optimizations we applied. Both optimizations are designed to avoid expensive external memory access.

\subsubsection{Maximized Feature Reuse}

\subsubsection{Optimized Datapath}
datapath that mitigate random access overhead, and avoid external memory access
